Towards a complete $A_4 \times SU(5)$ SUSY GUT

We propose a renormalisable model based on $A_4$ family symmetry with an $SU(5)$ grand unified theory (GUT) which leads to the minimal supersymmetric standard model (MSSM) with a two right-handed neutrino seesaw mechanism. Discrete $\mathbb{Z}_9\times \mathbb{Z}_6$ symmetry provides the fermion mass hierarchy in both the quark and lepton sectors, while $\mathbb{Z}_4^R$ symmetry is broken to $\mathbb{Z}_2^R$, identified as usual R-parity. Proton decay is highly suppressed by these symmetries. We discuss both the $A_4$ and $SU(5)$ symmetry breaking sectors, including doublet-triplet splitting, Higgs mixing and the origin of the $\mu$ term. The model provides an excellent fit (better than one sigma) to all quark and lepton (including neutrino) masses and mixing with spontaneous CP violation. With the $A_4$ vacuum alignments, $(0,1,1)$ and $(1,3,1)$, the model predicts the entire PMNS mixing matrix with no free parameters, up to a relative phase, selected to be $2\pi/3$ from a choice of the nine complex roots of unity, providing a direct link between neutrino oscillations and leptogenesis.

==> table_data.tex <==
\begingroup
\newcommand{\exto}[1]{{\smaller$ \times 10^{#1} $}}
\newcommand{\degr}{$^\circ$}

\begin{table}[ht]
\centering
\footnotesize
\begin{tabular}{| c | c c | c c |}
\hline
\multirow{2}{*}{\makecell{Parameter \\ {\scriptsize (from \cite{Antusch:2013jca})}}}	& \multicolumn{2}{c|}{\rule{0pt}{3ex}$ \tan \beta = 5 $} & \multicolumn{2}{c|}{$ \tan \beta = 10 $} \\[0.5ex]
\cline{2-5}
				& $ \mu_i $ & $ \Delta^\sigma_i $ & $ \mu_i $ & $ \Delta^\sigma_i $ \\
\hline \hline
\rule{0pt}{3ex}%
$\theta^q_{12}$ 		& 13.027\degr 	& 0.0814\degr 		& 13.027\degr 	& 0.0814\degr 	\\
$\theta^q_{13}$ 		& 0.1802\degr 	& 0.0281\degr 		& 0.1802\degr 	& 0.0281\degr 	\\
$\theta^q_{23}$ 		& 2.054\degr 	& 0.384\degr		& 2.054\degr 	& 0.384\degr	\\
$\delta^q$ 			& 69.21\degr	& 6.19\degr 		& 69.21\degr	& 6.19\degr 	\\
\rule{0pt}{3ex}%
$y_u$				& 2.92 \exto{-6} & 1.81 \exto{-6}	& 2.88 \exto{-6} & 1.79 \exto{-6} \\
$y_c$				& 1.43 \exto{-3} & 1.00 \exto{-4}	& 1.41 \exto{-3} & 9.87 \exto{-5} \\
$y_t$				& 5.34 \exto{-1} & 3.41 \exto{-2}	& 5.20 \exto{-1} & 3.15 \exto{-2} \\
\rule{0pt}{3ex}%
$y_d$				& 4.81 \exto{-6} & 1.06 \exto{-6}	& 4.84 \exto{-6} & 1.07 \exto{-6} \\
$y_s$				& 9.52 \exto{-5} & 1.03 \exto{-5}	& 9.59 \exto{-5} & 1.04 \exto{-5} \\
$y_b$				& 6.95 \exto{-3} & 1.75 \exto{-4}	& 7.01 \exto{-3} & 1.78 \exto{-4} \\
\rule{0pt}{3ex}%
$y_e$				& 1.97 \exto{-6} & 2.36 \exto{-8}	& 1.98 \exto{-6} & 2.38 \exto{-8} \\
$y_\mu$			& 4.16 \exto{-4} & 4.97 \exto{-6}	& 4.19 \exto{-4} & 5.02 \exto{-6} \\
$y_\tau$			& 7.07 \exto{-3} & 7.27 \exto{-5}	& 7.15 \exto{-3} & 7.42 \exto{-5} \\
\hline
\end{tabular}
\caption{Best fit values for quark and charged lepton parameters when run to the GUT scale as calculated in \cite{Antusch:2013jca}, with the SUSY breaking scale set at 1 TeV. We have included an overall contribution from threshold corrections corresponding to $ \bar{\eta}_b = -0.225 $ which affects primarily the $ b $ quark Yukawa coupling $ y_b $. $ \mu_i $ represents the best-fit value and $ \Delta^\sigma_i $ the $ 1\sigma $ error range, as defined in Eq.~\ref{eq:chisq}.}
\label{tab:data}
\end{table}

\begin{table}[ht]
\centering
\footnotesize
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{| c | r r | }
\hline
\rule{0pt}{4ex}\makecell{Parameter \\ {\scriptsize (from \cite{Gonzalez-Garcia:2014bfa})}}
						& \(\mu_i \pm1\sigma\) & 3\(\sigma\) range \\[1.5ex] \hline\hline
% \multicolumn{1}{| c |}{\( \sin^2 \theta_{12} \)}			& 0.304\(^{+0.013}_{-0.012}\)		& 0.270 \(\rightarrow\) 0.344	\\
\( \theta^l_{12} \,(^\circ)\)			& 33.48 \(^{+0.78}_{-0.75}\)		& 31.29 \(\rightarrow\) 35.91	\\ 
% \multicolumn{1}{| c |}{\( \sin^2 \theta_{23} \)}			& 0.452\(^{+0.052}_{-0.028}\)		& 0.382 \(\rightarrow\) 0.643	\\ 
\( \theta^l_{23} \,(^\circ)\)			& 42.3 \(^{+3.0}_{-1.6}\)		& 38.2 \(\rightarrow\) 53.3 	\\ 
% \multicolumn{1}{| c |}{\( \sin^2 \theta_{13} \)}			& 0.0218\(^{+0.0010}_{-0.0010}\)	& 0.0186 \(\rightarrow\) 0.0250	\\ 
\( \theta^l_{13} \,(^\circ)\)			& 8.5 \(^{+0.20}_{-0.21}\)		& 7.85 \(\rightarrow\) 9.10 	\\ 
\( \delta^l \,(^\circ)\)			& 306 \(^{+39}_{-70}\)			& 0 \(\rightarrow\) 360		\\ [5pt]
\(\dfrac{\Delta m^2_{21}}{10^{-5}}\) eV\(^2\)	& 7.50 \(^{+0.19}_{-0.17}\)		& 7.02 \(\rightarrow\) 8.09	\\ [8pt]
\(\dfrac{\Delta m^2_{31}}{10^{-3}}\) eV\(^2\) 	& +2.457 \(^{+0.047}_{-0.047}\)	& +2.317 \(\rightarrow\) +2.607\\ [5pt]
\hline
\end{tabular}
\caption{Table of current best fits to experimental data for lepton mixing angles and neutrino masses case of normal mass squared ordering taken from \cite{Gonzalez-Garcia:2014bfa}, with 1\(\sigma\) and 3\(\sigma\) uncertainty ranges.}
\label{tab:lepdata}
\end{table}

\endgroup
